Optically tuned soliton dynamics in Bose-Einstein condensates within dark traps

This study investigates the formation and dynamics of solitons in Bose-Einstein condensates (BECs) within dark traps generated by two crossed Laguerre-Gaussian (LG) beams with varying azimuthal indices $\ell$. As the index $\ell$ increases, the potential transitions from a harmonic trap when $\ell = 1$ to a square-well potential for larger values of $\ell$. This transition allows us to study a range of soliton dynamics under different confinement conditions while maintaining the same BEC volume. Through the derivation of the Gross-Pitaevskii equation (GPE) and under these specific conditions in both one-dimensional (1D) and two-dimensional (2D) configurations, we explore the dynamics of solitons across multiple scenarios. The study examines two primary methods for solitons generation: the temporal modulation of the scattering length and the implementation of an initial potential barrier that is subsequently removed. The results indicate that the trap shape plays a critical role in the generation and interaction dynamics of solitons. In harmonic traps, solitons exhibit a behavior different from those observed in anharmonic traps, where the dynamics is significantly influenced by the azimuthal index of the trap. The ability to control soliton dynamics in BECs holds significant promise for applications in quantum technologies, precision sensing, and the exploration of fundamental quantum phenomena.

==> Bibliography.tex <==
@article{Anderson1995,
  title={Observation of Bose-Einstein Condensation in a dilute atomic vapor},
  author={M. H. Anderson and J. R. Ensher and M. R. Matthews and C. E. Wieman and E. A. Cornell},
  journal={Science},
  volume={269},
  pages={198},
  year={1995}
}

@article{Weber2003,
  title={Bose-Einstein Condensation of Cesium},
  author={T. Weber and J. Herbig and M. Mark and H. C. Nagerl and R. Grimm},
  journal={Science},
  volume={299},
  pages={232},
  year={2003}
}

@article{Davis1995,
  title={Bose-Einstein Condensation in a Gas of Sodium Atoms},
  author={K. B. Davis and M. O. Mewes and M. R. Andrews and N. J. van Druten and D. S. Durfee and D. M. Kurn and W. Ketterle},
  journal={Phys. Rev. Lett.},
  volume={75},
  pages={3969},
  year={1995}
}

@article{Bradley1995,
  title={Evidence of Bose-Einstein Condensation in an Atomic Gas with Attractive Interactions},
  author={C. C. Bradley and C. A. Sackett and J. J. Tollett and R. C. Hulet},
  journal={Phys. Rev. Lett.},
  volume={75},
  pages={1687},
  year={1995}
}

@article{Roati2007,
  title={Bose-Einstein Condensate with Tunable Interactions},
  author={G. Roati and M. Zaccanti and C. D’Errico and M. Modugno and A. Simoni and M. Inguscio and G. Modugno},
  journal={Phys. Rev. Lett.},
  volume={99},
  pages={010403},
  year={2007}
}

@article{Fried1998,
  title={Bose-Einstein Condensation of Atomic Hydrogen},
  author={D. G. Fried and T. C. Killian and L. Willmann and D. Landhuis and S. C. Moss and D. Kleppner and T. J. Greytak},
  journal={Phys. Rev. Lett.},
  volume={81},
  pages={3811},
  year={1998}
}

@article{Robert2001,
  title={A Bose-Einstein Condensate of Metastable Atoms},
  author={A. Robert and O. Sirjean and A. Browaeys and J. Poupard and S. Nowak and D. Boiron and C. I. Westbrook and A. Aspect},
  journal={Science},
  volume={292},
  pages={461},
  year={2001}
}

@article{Santos2001,
  title={Bose-Einstein Condensation of Metastable Helium},
  author={F. Pereira Dos Santos and J. Léonard and J. Wang and C. J. Barrelet and F. Perales and E. Rasel and C. S. Unnikrishnan and M. Leduc and C. Cohen-Tannoudji},
  journal={Phys. Rev. Lett.},
  volume={86},
  pages={3459},
  year={2001}
}

@article{Fukuhara2007,
  title={A Bose-Einstein Condensation of an Ytterbium Isotope},
  author={T. Fukuhara and S. Sugawa and Y. Takahashi},
  journal={Phys. Rev. A},
  volume={76},
  pages={051604},
  year={2007}
}

@article{Beaufils2008,
  title={All Optical Production of Chromium Bose-Einstein Condensates},
  author={Q. Beaufils and R. Chicireanu and T. Zanon and B. Laburthe-Tora and E. Maréchal and L. Vernac and J. C. Keller and O. Gorceix},
  journal={Phys. Rev. A},
  volume={77},
  pages={06160},
  year={2008}
}

@article{Griesmaier2005,
  title={Bose-Einstein Condensation of Chromium},
  author={A. Griesmaier and J. Werner and S. Hensler and J. Stuhler and T. Pfau},
  journal={Phys. Rev. Lett.},
  volume={94},
  pages={160401},
  year={2005}
}

@article{Jaouadi2010,
  title={Bose-Einstein condensation in dark power-law laser traps},
  author={A. Jaouadi and N. Gaaloul and B. Viaris de Lesegno and M. Telmini and L. Pruvost and E. Charron},
  journal={Phys. Rev. A},
  volume={82},
  pages={023613},
  year={2010}
}

@article{Mewes1997,
  title={Output Coupler for Bose-Einstein Condensed Atoms},
  author={M. O. Mewes and M. R. Andrews and D. M. Kurn and D. S. Durfee and C. G. Townsend and W. Ketterle},
  journal={Phys. Rev. Lett.},
  volume={78},
  pages={582},
  year={1997}
}

@article{Bloch1999,
  title={Atom Laser with a cw Output Coupler},
  author={I. Bloch and T. W. Hansch and T. Esslinger},
  journal={Phys. Rev. Lett.},
  volume={82},
  pages={3008},
  year={1999}
}

@article{Gaaloul2007,
  title={Optical devices for cold atoms and Bose-Einstein Condensates},
  author={N. Gaaloul and A. Jaouadi and L. Pruvost and M. Telmini and E. Charron},
  journal={American Institute of Physics Conference Proceedings},
  volume={935},
  pages={10},
  year={2007}
}

@article{Gaaloul2009,
  title={Controlled deflection of cold atomic clouds and of a Bose-Einstein Condensate},
  author={N. Gaaloul and A. Jaouadi and L. Pruvost and M. Telmini and E. Charron},
  journal={Eur. Phys. J. D},
  volume={53},
  pages={343},
  year={2009}
}

@article{khaykovich2002,
  title={Formation of a Matter-Wave Bright Soliton},
  author={Khaykovich, L and Schreck, F and Ferrari, G and Bourdel, T and Cubizolles, J and Carr, LD and Castin, Y and Salomon, C},
  journal={Science},
  volume={296},
  number={5571},
  pages={1290--1293},
  year={2002},
  publisher={American Association for the Advancement of Science}
}

@article{mollenauer1980,
  title={Experimental Observation of Picosecond Pulse Narrowing and Solitons in Optical Fibers},
  author={Mollenauer, LF and Stolen, RH and Gordon, JP},
  journal={Physical Review Letters},
  volume={45},
  number={13},
  pages={1095},
  year={1980},
  publisher={APS}
}

@article{wu1984observation,
  title={Observation of a Nonpropagating Hydrodynamic Soliton},
  author={Wu, Junru and Keolian, Robert and Rudnick, Isadore},
  journal={Physical Review Letters},
  volume={52},
  number={16},
  pages={1421},
  year={1984},
  publisher={APS}
}

@article{kosevich1990magnetic,
  title={Magnetic Solitons},
  author={Kosevich, AM and Ivanov, BA and Kovalev, AS},
  journal={Physics Reports},
  volume={194},
  number={3},
  pages={117--238},
  year={1990},
  publisher={Elsevier}
}

@article{tanaka2001soliton,
  title={Soliton in Two-Band Superconductor},
  author={Tanaka, Y},
  journal={Physical Review Letters},
  volume={88},
  number={1},
  pages={017002},
  year={2001},
  publisher={APS}
}

@article{allen1992orbital,
  title={Orbital angular momentum of light and the transformation of Laguerre-Gaussian laser modes},
  author={Allen, L and Beijersbergen, MW and Spreeuw, RJ and Woerdman, JP},
  journal={Physical Review A},
  volume={45},
  number={11},
  pages={8185},
  year={1992},
  publisher={APS}
}

@article{denschlag2000,
  title={Generating solitons by phase engineering of a Bose-Einstein condensate},
  author={Denschlag, J and Simsarian, JE and Feder, DL and Clark, CW and Collins, LA and Cubizolles, J and Deng, L and Hagley, EW and Helmerson, K and Reinhardt, WP},
  journal={Science},
  volume={287},
  number={5450},
  pages={97--101},
  year={2000},
  publisher={American Association for the Advancement of Science}
}

@article{Alison2022,
  title = {Control of Light-Atom Solitons and Atomic Transport by Optical Vortex Beams Propagating through a Bose-Einstein Condensate},
  author = {Henderson, Grant W. and Robb, Gordon R. M. and Oppo, Gian-Luca and Yao, Alison M.},
  journal = {Phys. Rev. Lett.},
  volume = {129},
  issue = {7},
  pages = {073902},
  numpages = {5},
  year = {2022},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.129.073902},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.129.073902}
}

@article{Yang23,
author = {Mingyue Yang and Guochao Wang and Zhichuang Wang and Xianbin Li and Lingxiao Zhu and Weiqiang Wang and Wenfu Zhang and Shuhua Yan and Jun Yang},
journal = {Opt. Lett.},
keywords = {Absolute distance measurement; Beam splitters; Frequency modulation; Interferometers; Laser sources; Phase measurement},
number = {16},
pages = {4356--4359},
publisher = {Optica Publishing Group},
title = {Micrometer-precision absolute distance measurement with a repetition-rate-locked soliton microcomb},
volume = {48},
month = {Aug},
year = {2023},
url = {https://opg.optica.org/ol/abstract.cfm?URI=ol-48-16-4356},
doi = {10.1364/OL.499291}
}

@book{Hirota,
    author ={R. Hirota} ,
    title = {The Direct Method in Soliton Theory},
    publisher = {Cambridge University Press},
    year ={2004} 
}

@article{MORALES2022,
title = {Quantum sensing of matter waves using BEC oscillations},
journal = {Results in Physics},
volume = {41},
pages = {105923},
year = {2022},
issn = {2211-3797},
doi = {https://doi.org/10.1016/j.rinp.2022.105923},
url = {https://www.sciencedirect.com/science/article/pii/S2211379722005472},
author = {L. Morales-Molina and E. Arévalo},
keywords = {Bose–Einstein in optical lattices, Tunneling of atoms, Sensing, Solitons},
}

@article{eiermann2004,
  title={Bright Bose-Einstein Gap Solitons of Atoms with Repulsive Interaction},
  author={Eiermann, B and Anker, Th and Albiez, M and Taglieber, M and Treutlein, P and Marzlin, KP and Oberthaler, MK},
  journal={Physical Review Letters},
  volume={92},
  number={23},
  pages={230401},
  year={2004},
  publisher={APS}
}

@misc{Henderson2020,
  title={Data for: "Control of light-atom solitons and atomic transport by optical vortex beams propagating through a Bose-Einstein Condensate"},
  author={G. Henderson and G. R. M. Robb and G.-L. Oppo and A. M. Yao},
  note={University of Strathclyde KnowledgeBase},
  year={2020}
}

@article{David2012,
  title = {Coherent emission of atomic soliton pairs by Feshbach-resonance tuning},
  author = {Michinel, Humberto and Paredes, \'Angel and Valado, Mar\'{\i}a M. and Feijoo, David},
  journal = {Phys. Rev. A},
  volume = {86},
  issue = {1},
  pages = {013620},
  numpages = {7},
  year = {2012},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.86.013620},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.86.013620}
}

@article{Strecker2002,
  author    = {K. E. Strecker and G. B. Partridge and A. G. Truscott and R. G. Hulet},
  title     = {Formation and propagation of matter-wave soliton trains},
  journal   = {Nature},
  volume    = {417},
  pages     = {150--153},
  year      = {2002},
  doi       = {10.1038/nature747},
}

@article{Wang,
    author = {H. Wang, Q. Zhou and W. Liu},
    title = {Exact analysis and elastic interaction of multi-soliton for a two-dimensional Gross-Pitaevskii equation in the Bose-Einstein condensation},
    journal = {Journal of Advanced Research},
    volume={38},
    pages={179-190},
    year = {2022}
}

@article{Cornish2006,
  author    = {S. L. Cornish and S. T. Thompson and C. E. Wieman},
  title     = {Formation of Bright Matter-Wave Solitons during the Collapse of Attractive Bose-Einstein Condensates},
  journal   = {Phys. Rev. Lett.},
  volume    = {96},
  pages     = {170401},
  year      = {2006},
  doi       = {10.1103/PhysRevLett.96.170401},
}

@article{Nguyen2014,
  author    = {J. H. V. Nguyen and P. Dyke and D. Luo and B. A. Malomed and R. G. Hulet},
  title     = {Collisions of Matter-Wave Solitons},
  journal   = {Nature Physics},
  volume    = {10},
  pages     = {918--922},
  year      = {2014},
  doi       = {10.1038/nphys3135},
}

@misc{nobel2001,
  author       = {Nobel Prize Outreach AB},
  title        = {The Nobel Prize in Physics 2001},
  year         = {2024},
  note         = {NobelPrize.org. Fri. 19 Jul 2024},
  howpublished = {\url{https://www.nobelprize.org/prizes/physics/2001/summary/}}
}

@article{Carretero-Gonzalez2008,
author = {Carretero-Gonzalez, Ricardo and Frantzeskakis, D. and Kevrekidis, P.},
year = {2008},
month = {07},
pages = {},
title = {INVITED ARTICLE: Nonlinear waves in Bose Einstein condensates: physical relevance and mathematical techniques},
volume = {21},
journal = {Nonlinearity},
doi = {10.1088/0951-7715/21/7/R01}
}

@article{2019_Hussain,
author = {Jameel Hussain and Javed Akram and FARHAN SAIF},
title = {Gray and Dark Soliton Behavior and Population Under a Symmetric and Asymmetric Potential Trap},
journal = {Journal of Low Temperature Physics},
year = {2019},
volume = {195},
publisher = {Springer Nature},
month = {mar},
url = {https://doi.org/10.1007/s10909-019-02172-z},
number = {5-6},
pages = {429--436},
doi = {10.1007/s10909-019-02172-z}
}

@article{Inouye1998,
  title = {Observation of Feshbach resonances in a Bose–Einstein condensate},
  author = {Inouye, S. and Andrews, M. R. and Stenger, J. and Miesner, H.-J. and Stamper-Kurn, D. M. and Ketterle, W.},
  journal = {Nature},
  volume = {392},
  number = {6672},
  pages = {151-154},
  year = {1998}
}

@article{Chin2010,
  title = {Feshbach resonances in ultracold gases},
  author = {Chin, C. and Grimm, R. and Julienne, P. and Tiesinga, E.},
  journal = {Reviews of Modern Physics},
  volume = {82},
  number = {2},
  pages = {1225},
  year = {2010}
}

@article{Burger1999,
  title = {Dark solitons in Bose-Einstein condensates},
  author = {Burger, S. and Bongs, K. and Dettmer, S. and Ertmer, W. and Sengstock, K. and Sanpera, A. and Shlyapnikov, G. V. and Lewenstein, M.},
  journal = {Physical Review Letters},
  volume = {83},
  number = {25},
  pages = {5198},
  year = {1999}
}

@article{Anderson2001,
  title = {Watching dark solitons decay into vortex rings in a Bose-Einstein condensate},
  author = {Anderson, B. P. and Denschlag, J. H. and Haffner, H. and Antonakis, C. and Hagley, E. W. and Hellweg, D. and Rolston, S. L. and Phillips, W. D.},
  journal = {Physical Review Letters},
  volume = {86},
  number = {14},
  pages = {2926},
  year = {2001}
}


@article{Kosloff1986,
  author    = {R. Kosloff and H. Tal-Ezer},
  title     = {A direct relaxation method for calculating eigenfunctions and eigenvalues of the Schrödinger equation on a grid},
  journal   = {Chem. Phys. Lett.},
  year      = {1986},
  volume    = {127},
  pages     = {223-230}
}

@article{Brachmann11,
author = {J. F. S. Brachmann and W. S. Bakr and J. Gillen and A. Peng and M. Greiner},
journal = {Opt. Express},
keywords = {Coherent optical effects; Multiphoton processes; Binary optics; Diffractive optics; Atom optics ; Bose-Einstein condensates ; Optical vortices ; Bose Einstein condensates; Laser beams; Light beams; Optical vortices; Orbital angular momentum multiplexing; Two level systems},
number = {14},
pages = {12984--12991},
publisher = {Optica Publishing Group},
title = {Inducing vortices in a Bose-Einstein condensate using holographically produced light beams},
volume = {19},
month = {Jul},
year = {2011},
url = {https://opg.optica.org/oe/abstract.cfm?URI=oe-19-14-12984},
doi = {10.1364/OE.19.012984},

}

@article{marchant2013,
  title={Controlled formation and reflection of a bright solitary matter-wave},
  author={Marchant, Annabel L and Billam, Thomas P and Wiles, Tom P and Yu, Ming Mei and Gardiner, Simon A and Cornish, Simon L},
  journal={Nature Communications},
  volume={4},
  pages={1865},
  year={2013},
  publisher={Nature Publishing Group}
}

@article{carr2002,
  title={Dynamics of a matter-wave bright soliton in an expulsive potential},
  author={Carr, Lincoln D and Castin, Yvan},
  journal={Physical Review A},
  volume={66},
  number={6},
  pages={063602},
  year={2002},
  publisher={American Physical Society}
}




